Multi-task twin support vector machine with Universum data

Multi-task learning (MTL) has emerged as a promising topic of machine learning in recent years, aiming to enhance the performance of numerous related learning tasks by exploiting beneficial information. During the training phase, most of the existing multi-task learning models concentrate entirely on the target task data and ignore the non-target task data contained in the target tasks. To address this issue, Universum data, that do not correspond to any class of a classification problem, may be used as prior knowledge in the training model. This study looks at the challenge of multi-task learning using Universum data to employ non-target task data, which leads to better performance. It proposes a multi-task twin support vector machine with Universum data (UMTSVM) and provides two approaches to its solution. The first approach takes into account the dual formulation of UMTSVM and tries to solve a quadratic programming problem. The second approach formulates a least-squares version of UMTSVM and refers to it as LS-UMTSVM to further increase the generalization performance. The solution of the two primal problems in LS-UMTSVM is simplified to solving just two systems of linear equations, resulting in an incredibly simple and quick approach. Numerical experiments on several popular multi-task data sets and medical data sets demonstrate the efficiency of the proposed methods.

==> references.tex <==
@article{xie2015multitask,
	title={Multitask centroid twin support vector machines},
	author={Xie, Xijiong and Sun, Shiliang},
	journal={Neurocomputing},
	volume={149},
	pages={1085--1091},
	year={2015},
	publisher={Elsevier}
}
@inproceedings{xie2012multitask,
	title={Multitask twin support vector machines},
	author={Xie, Xijiong and Sun, Shiliang},
	booktitle={International Conference on Neural Information Processing},
	pages={341--348},
	year={2012},
	organization={Springer}
}
@article{khemchandani2007twin,
 author = "Jayadeva and R. Khemchandani and S. Chandra",
 title = "Twin support vector machines for pattern classification",
 journal = "IEEE Transactions on Pattern Analysis and Machine Intelligence",
 volume = "29",
 number = "5",
 pages = "905-910",
 year = "2007",
}
@article{mangasarian2005multisurface,
 author = "Mangasarian, Olvi L and Wild, Edward W",
 title = "Multisurface proximal support vector machine classification via generalized eigenvalues",
 sjournal = " IEEE Trans. Pattern Anal. Mach. Intell.",
 journal = "IEEE Transactions on Pattern Analysis and Machine Intelligence",
 volume = "28",
 number = "1",
 pages = "69-74",
 year = "2006",
}
@article{xu2016nu,
	title={$\nu$-twin support vector machine with universum data for classification},
	author={Xu, Yitian and Chen, Mei and Yang, Zhiji and Li, Guohui},
	journal={Applied Intelligence},
	volume={44},
	number={4},
	pages={956--968},
	year={2016},
	publisher={Springer}
}
@article{xiao2021new,
	title={A new multi-task learning method with universum data},
	author={Xiao, Yanshan and Wen, Jing and Liu, Bo},
	journal={Applied Intelligence},
	volume={51},
	number={6},
	pages={3421--3434},
	year={2021},
	publisher={Springer}
}
@article{moosaei2021universum,
	title={Universum parametric-margin $\nu$-support vector machine for classification using the difference of convex functions algorithm},
	author={Moosaei, Hossein and Bazikar, Fatemeh and Ketabchi, Saeed and Hlad{\'\i}k, Milan},
	journal={Applied Intelligence},
	pages={1--21},
	year={2021},
	publisher={Springer}
}

@article{richhariya2018eeg,
 author = {Richhariya, Bharat and Tanveer, Muhammad},
 title = {{EEG} signal classification using universum support vector machine},
 journal = {Expert Systems with Applications},
 volume = {106},
 pages = {169-182},
 year = {2018},
}
@article{bakker2003task,
 author={Bakker, Bart and Heskes, Tom},
 title={Task clustering and gating for bayesian multitask learning},
 journal={Journal of Machine Learning Research},
 volume={4},
 year={2003},
}
@article{ando2005framework,
	title={A framework for learning predictive structures from multiple tasks and unlabeled data.},
	author={Ando, Rie Kubota and Zhang, Tong and Bartlett, Peter},
	journal={Journal of Machine Learning Research},
	volume={6},
	number={11},
	year={2005}
}
@inproceedings{bi2008improved,
	title={An improved multi-task learning approach with applications in medical diagnosis},
	author={Bi, Jinbo and Xiong, Tao and Yu, Shipeng and Dundar, Murat and Rao, R Bharat},
	booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
	pages={117--132},
	year={2008},
	organization={Springer}
}
@article{birlutiu2010multi,
	title={Multi-task preference learning with an application to hearing aid personalization},
	author={Birlutiu, Adriana and Groot, Perry and Heskes, Tom},
	journal={Neurocomputing},
	volume={73},
	number={7-9},
	pages={1177--1185},
	year={2010},
	publisher={Elsevier}
}
@inproceedings{chapelle2010multi,
	title={Multi-task learning for boosting with application to web search ranking},
	author={Chapelle, Olivier and Shivaswamy, Pannagadatta and Vadrevu, Srinivas and Weinberger, Kilian and Zhang, Ya and Tseng, Belle},
	booktitle={Proceedings of the 16th ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={1189--1198},
	year={2010}
}
@article{ren2016multicell,
	title={A multiCell visual tracking algorithm using multi-task particle swarm optimization for low-contrast image sequences},
	author={Ren, Yayun and Xu, Benlian and Zhu, Peiyi and Lu, Mingli and Jiang, Dongmei},
	journal={Applied Intelligence},
	volume={45},
	number={4},
	pages={1129--1147},
	year={2016},
	publisher={Springer}
}
@article{zhou2018position,
 author={Zhou, Deyu and Miao, Lei and He, Yulan},
 title={Position-aware deep multi-task learning for drug--drug interaction extraction},
 journal={Artificial Intelligence in Medicine},
 volume={87},
 pages={1-8},
 year={2018},
}
@article{su2017multi,
 author={Su, Chi and Yang, Fan and Zhang, Shiliang and Tian, Qi and Davis, Larry Steven and Gao, Wen},
 title={Multi-task learning with low rank attribute embedding for multi-camera person re-identification},
 journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
 volume={40},
 number={5},
 pages={1167-1181},
 year={2017},
}
@article{cheng2015multi,
	title={Multi-task object tracking with feature selection},
	author={Cheng, Xu and Li, Nijun and Zhou, Tongchi and Wu, Zhenyang and Zhou, Lin},
	journal={IEICE Transactions on Fundamentals of Electronics, Communications and Computer Sciences},
	volume={98},
	number={6},
	pages={1351--1354},
	year={2015},
	publisher={The Institute of Electronics, Information and Communication Engineers}
}




@article{mei2020multi,
	title={Multi-task $\nu$-twin support vector machines},
	author={Mei, Benshan and Xu, Yitian},
	journal={Neural Computing and Applications},
	volume={32},
	number={15},
	pages={11329--11342},
	year={2020},
	publisher={Springer}
}
@article{shao2011improvements,
 author = {Shao, Yuan-Hai and Zhang, Chun-Hua and Wang, Xiao-Bo and Deng, Nai-Yang},
 title = {Improvements on twin support vector machines},
 journal = {IEEE Transactions on Neural Networks},
 volume = {22},
 number = {6},
 pages = {962--968},
 year = {2011},
}

@article{lu2018svm,
 author={Lu, Liyun and Lin, Qiang and Pei, Huimin and Zhong, Ping},
 title={The {aLS}-{SVM} based multi-task learning classifiers},
 journal={Applied Intelligence},
 volume={48},
 number={8},
 pages={2393-2407},
 year={2018},
}

@incollection{vapnik200624,
 author = {Vapnik, Vladimir},
 title={Transductive Inference and Semi-Supervised Learning},
 editor = {Olivier Chapelle and Bernhard Sch\"{o}lkopf and Alexander Zien},
 booktitle = {Semi-Supervised Learning},
 publisher = {MIT Press},
 pages = {453-472}, 
 year = {2006},
}
@book{vapnik2006estimation,
 title = {Estimation of Dependences Based on Empirical Data},
 author = {Vapnik, Vladimir},
 publisher = {Springer},
 address = {New York},
 year = {2006},
}

@inproceedings{zhang2008semi,
	title={Semi-supervised classification with universum},
	author={Zhang, Dan and Wang, Jingdong and Wang, Fei and Zhang, Changshui},
	booktitle={Proceedings of the 2008 SIAM International Conference on Data Mining},
	pages={323--333},
	year={2008},
	organization={SIAM}
}
@article{chapelle2007analysis,
 author = "Chapelle, Olivier and Agarwal, Alekh and Sinz, Fabian and Sch{\"o}lkopf, Bernhard",
  title = "An analysis of inference with the universum",
  journal = "Advances in Neural Information Processing Systems",
  volume = "20",
  pages = "1369-1376",
  year = "2007",
}
@article{kumar2009least,
 author={Kumar, M Arun and Gopal, Madan},
 title={Least squares twin support vector machines for pattern classification},
 journal={Expert Systems with Applications},
 volume={36},
 number={4},
 pages={7535-7543},
 year={2009},
}

@article{ji2013multitask,
	title={Multitask multiclass support vector machines: model and experiments},
	author={Ji, You and Sun, Shiliang},
	journal={Pattern Recognition},
	volume={46},
	number={3},
	pages={914--924},
	year={2013},
	publisher={Elsevier}
}
@inproceedings{shiao2012implementation,
 author={Shiao, Han-Tai and Cherkassky, Vladimir},
 title={Implementation and comparison of {SVM}-based multi-task learning methods},
 booktitle={The 2012 International Joint Conference on Neural Networks (IJCNN)},
 pages={1-7},
 year={2012},
 organization={IEEE},
}
@inproceedings{xue2016multi,
 author={Xue, Yongjian and Beauseroy, Pierre},
 title={Multi-task learning for one-class {SVM} with additional new features},
 booktitle={2016 23rd International Conference on Pattern Recognition (ICPR)},
 pages={1571-1576},
 year={2016},
 organization={IEEE},
}
@inproceedings{yang2010multi,
	title={Multi-task learning for one-class classification},
	author={Yang, Haiqin and King, Irwin and Lyu, Michael R},
	booktitle={The 2010 International Joint Conference on Neural Networks (IJCNN)},
	pages={1--8},
	year={2010},
	organization={IEEE}
}
@inproceedings{evgeniou2004regularized,
	title={Regularized multi--task learning},
	author={Evgeniou, Theodoros and Pontil, Massimiliano},
	booktitle={Proceedings of the tenth ACM SIGKDD international conference on Knowledge discovery and data mining},
	pages={109--117},
	year={2004}
}

@article{moosaei2021generalized,
	title={Generalized Twin Support Vector Machines},
	author={Moosaei, Hossein and Ketabchi, Saeed and Razzaghi, Mohamad and Tanveer, Muhammad},
	journal={Neural Processing Letters},
	volume={53},
	number={2},
	pages={1545--1564},
	year={2021},
	publisher={Springer}
}
@article{zhang2013mixed,
	title={Mixed-norm linear support vector machine},
	author={Zhang, Chunhua and Shao, Yuanhai and Tan, Junyan and Deng, Naiyang},
	journal={Neural Computing and Applications},
	volume={23},
	number={7},
	pages={2159--2166},
	year={2013},
	publisher={Springer}
}





@article{wright1999numerical,
	title={Numerical optimization},
	author={Wright, Stephen and Nocedal, Jorge},
	journal={Springer Science},
	volume={35},
	number={67-68},
	pages={7},
	year={1999}
}
@inproceedings{richhariya2018improved,
 author = {Richhariya, Bharat and Sharma, Abhinav and Tanveer, Muhammad},
 title = {Improved universum twin support vector machine},
 editor = {Suresh Sundaram},
 booktitle = {2018 IEEE Symposium Series on Computational Intelligence (IEEE SSCI 2018)},
 pages = {2045-2052},
 year = {2018},
 publisher = {IEEE},
}




@article{richhariya2020reduced,
	title={A reduced universum twin support vector machine for class imbalance learning},
	author={Richhariya, Bharat and Tanveer, Muhammad},
	journal={Pattern Recognition},
	volume={102},
	pages={107150},
	year={2020},
	publisher={Elsevier}
}
@inproceedings{zhang2020sparse,
 author = {Zhang, Xiaoou and Zhu, Zexuan},
 title = {Sparse Multi-task Least-Squares Support Vector Machine},
 editor = {Zhang, Haijun and Zhang, Zhao and Wu, Zhou and Hao, Tianyong},
 booktitle = {Neural Computing for Advanced Applications, NCAA 2020},
 series = {CCIS},
 fseries = {Communications in Computer and Information Science},
 volume = {1265},
 address = {Singapore},
 publisher = {Springer},
 pages = {157-167},
 year = {2020},
}
@article{li2021dc,
 title = {{DC} programming for sparse proximal support vector machines},
 author = {Li, Guoquan and Yang, Linxi and Wu, Zhiyou and Wu, Changzhi},
 journal = {Information Sciences},
 volume  ={547},
 pages = {187-201},
 year = {2021},
}
@inproceedings{tanveer2019improved,
 title = {Improved sparse pinball twin {SVM}},
 author = {Tanveer, Muhammad and Rajani, T and Ganaie, M A},
 editor = {Shun-Feng Su},
 booktitle = {2019 IEEE International Conference on Systems, Man and Cybernetics (SMC)},
 location = {Bari, Italy},
 pages = {3287-3291},
 year = {2019},
 publisher={IEEE},
}
@article{tanveer2021sparse,
	title={Sparse Twin Support Vector Clustering using Pinball Loss},
	author={Tanveer, M and Gupta, Tarun and Shah, Miten and Richhariya, Bharat},
	journal={IEEE Journal of Biomedical and Health Informatics},
	year={2021},
	publisher={IEEE}
}
@article{tanveer2019sparse,
	title={Sparse pinball twin support vector machines},
	author={Tanveer, Muhammad and Tiwari, Aruna and Choudhary, Rahul and Jalan, Sanchit},
	journal={Applied Soft Computing},
	volume={78},
	pages={164--175},
	year={2019},
	publisher={Elsevier}
}
@article{moosaei2021sparse,
	title={Sparse Universum Quadratic Surface Support Vector Machine Models for Binary Classification},
	author={Moosaei, Hossein and Mousavi, Ahmad and Hlad{\'\i}k, Milan and Gao, Zheming},
	journal={arXiv preprint arXiv:2104.01331},
	year={2021}
}
@article{zhang2013mixed,
	title={Mixed-norm linear support vector machine},
	author={Zhang, Chunhua and Shao, Yuanhai and Tan, Junyan and Deng, Naiyang},
	journal={Neural Computing and Applications},
	volume={23},
	number={7},
	pages={2159--2166},
	year={2013},
	publisher={Springer}
}
@article{tan2014laplacian,
	title={Laplacian p-norm proximal support vector machine for semi-supervised classification},
	author={Tan, Junyan and Zhen, Ling and Deng, Naiyang and Zhang, Zhiqiang},
	journal={Neurocomputing},
	volume={144},
	pages={151--158},
	year={2014},
	publisher={Elsevier}
}
@article{zhang2014sparse,
	title={Sparse least square twin support vector machine with adaptive norm},
	author={Zhang, Zhiqiang and Zhen, Ling and Deng, Naiyang and Tan, Junyan},
	journal={Applied intelligence},
	volume={41},
	number={4},
	pages={1097--1107},
	year={2014},
	publisher={Springer}
}
@article{chen2020nprsvm,
 author={Chen, Wei-Jie and Shao, Yuan-Hai and Li, Chun-Na and Wang, Yu-Qing and Liu, Ming-Zeng and Wang, Zhen},
 title={{NPrSVM}: Nonparallel sparse projection support vector machine with efficient algorithm},
 journal={Applied Soft Computing},
 volume={90},
 pages={106142},
 year={2020},
}
@article{ketabchi2019improvement,
  title={An improvement on parametric  $\nu$-support vector algorithm for classification},
  author={Ketabchi, Saeed and Moosaei, Hossein and Razzaghi, Mohamad and Pardalos, Panos M},
  journal={Annals of Operations Research},
  volume={276},
  number={1},
  pages={155--168},
  year={2019},
  publisher={Springer}
}
@article{pappu2015sparse,
	title={Sparse proximal support vector machines for feature selection in high dimensional datasets},
	author={Pappu, Vijay and Panagopoulos, Orestis P and Xanthopoulos, Petros and Pardalos, Panos M},
	journal={Expert Systems with Applications},
	volume={42},
	number={23},
	pages={9183--9191},
	year={2015},
	publisher={Elsevier}
}
@article{peng2010nu,
 author = {Peng, Xinjun},
 title = {A $\nu$-twin support vector machine ($\nu$-{TSVM}) classifier and its geometric algorithms},
 journal = {Information Sciences},
 volume = {180},
 number = {20},
 pages = {3863-3875},
 year = {2010},
}
@article{peng2010tsvr,
 author = {Peng, Xinjun},
 title = {{TSVR}: an efficient twin support vector machine for regression},
 journal = {Neural Networks},
 volume = {23},
 number = {3},
 pages = {365-372},
 year = {2010},
}
@article{wang2020wavelet,
	title={Wavelet transform-based weighted $\nu$-twin support vector regression},
	author={Wang, Lidong and Gao, Chuang and Zhao, Nannan and Chen, Xuebo},
	journal={International Journal of Machine Learning and Cybernetics},
	volume={11},
	number={1},
	pages={95--110},
	year={2020},
	publisher={Springer}
}
@article{maldonado2011simultaneous,
  title={Simultaneous feature selection and classification using kernel-penalized support vector machines},
  author={Maldonado, Sebasti{\'a}n and Weber, Richard and Basak, Jayanta},
  journal={Information Sciences},
  volume={181},
  number={1},
  pages={115--128},
  year={2011},
  publisher={Elsevier}
}
@article{chandrashekar2014survey,
  title={A survey on feature selection methods},
  author={Chandrashekar, Girish and Sahin, Ferat},
  journal={Computers \& Electrical Engineering},
  volume={40},
  number={1},
  pages={16--28},
  year={2014},
  publisher={Elsevier}
}
@article{liu2015semi,
 author={Liu, Chien-Liang and Hsaio, Wen-Hoar and Lee, Chia-Hoang and Chang, Tao-Hsing and Kuo, Tsung-Hsun},
 title={Semi-supervised text classification with universum learning},
 journal={IEEE Transactions on Cybernetics},
 volume={46},
 number={2},
 pages={462-473},
 year={2015},
}
@article{li2019classification,
  title={Classification of heart sounds based on the wavelet fractal and twin support vector machine},
  author={Li, Jinghui and Ke, Li and Du, Qiang},
  journal={Entropy},
  volume={21},
  number={5},
  pages={472},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}
@article{chen2016sparse,
  title={Sparse solutions of linear complementarity problems},
  author={Chen, Xiaojun and Xiang, Shuhuang},
  journal={Mathematical Programming},
  volume={159},
  number={1},
  pages={539--556},
  year={2016},
  publisher={Springer}
}

@article{peng2010least,
 author = {Peng, Xinjun},
 title = {Least squares twin support vector hypersphere {(LS-TSVH)} for pattern recognition},
 journal = {Expert Systems with Applications},
 volume = {37},
 number = {12},
 pages = {8371-8378},
 year = {2010},
}
@article{kumar2008application,
	title={Application of smoothing technique on twin support vector machines},
	author={Kumar, M Arun and Gopal, Madan},
	journal={Pattern Recognition Letters},
	volume={29},
	number={13},
	pages={1842--1848},
	year={2008},
	publisher={Elsevier}
}
@article{khemchandani2009optimal,
	title={Optimal kernel selection in twin support vector machines},
	author={Khemchandani, Reshma and Chandra, Suresh and others},
	journal={Optimization Letters},
	volume={3},
	number={1},
	pages={77--88},
	year={2009},
	publisher={Springer}
}
@article{shao2013least,
	title={Least squares twin parametric-margin support vector machine for classification},
	author={Shao, Yuan-Hai and Wang, Zhen and Chen, Wei-Jie and Deng, Nai-Yang},
	journal={Applied intelligence},
	volume={39},
	number={3},
	pages={451--464},
	year={2013},
	publisher={Springer}
}

@article{khemchandani2011generalized,
	title={Generalized eigenvalue proximal support vector regressor},
	author={Khemchandani, Reshma and Karpatne, Anuj and Chandra, Suresh},
	journal={Expert Systems with Applications},
	volume={38},
	number={10},
	pages={13136--13142},
	year={2011},
	publisher={Elsevier}
}
@article{akyildirim2021prediction,
  title={Prediction of cryptocurrency returns using machine learning},
  author={Akyildirim, Erdinc and Goncu, Ahmet and Sensoy, Ahmet},
  journal={Annals of Operations Research},
  volume={297},
  number={1},
  pages={3--36},
  year={2021},
  publisher={Springer}
}
@article{arabasadi2017computer,
 author = {Arabasadi, Zeinab and Alizadehsani, Roohallah and Roshanzamir, Mohamad and Moosaei, Hossein and Yarifard, Ali Asghar},
 title = {Computer aided decision making for heart disease detection using hybrid neural network-{Genetic} algorithm},
 journal = {Computer Methods and Programs in Biomedicine},
 volume = {141},
 pages = {19--26},
 year = {2017},
}

@article{cai2004application,
 author = {Cai, Yu-Dong and Ricardo, Pong-Wong and Jen, Chih-Hung and Chou, Kuo-Chen},
 title = {Application of {SVM} to predict membrane protein types},
 journal = {Journal of Theoretical Biology},
 volume = {226},
 number = {4},
 pages = {373--376},
 year = {2004},
}
@article{javadi2019learning,
  title={Learning wireless sensor networks for source localization},
  author={Javadi, S Hamed and Moosaei, Hossein and Ciuonzo, Domenico},
  journal={Sensors},
  volume={19},
  number={3},
  pages={635},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}
@article{guarracino2007classification,
  title={A classification method based on generalized eigenvalue problems},
  author={Guarracino, Mario Rosario and Cifarelli, Claudio and Seref, Onur and Pardalos, Panos M},
  journal={Optimisation Methods and Software},
  volume={22},
  number={1},
  pages={73--81},
  year={2007},
  publisher={Taylor \& Francis}
}
@article{wang2011color,
  title={Color image segmentation using pixel wise support vector machine classification},
  author={Wang, Xiang-Yang and Wang, Ting and Bu, Juan},
  journal={Pattern Recognition},
  volume={44},
  number={4},
  pages={777--787},
  year={2011},
  publisher={Elsevier}
}
@article{duncan1944lxxviii,
  title={Some devices for the solution of large sets of simultaneous linear equations. ({With} an appendix on the reciprocation of partitioned matrices)},
  author={Duncan, William Jolly},
  journal={The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
  volume={35},
  number={249},
  pages={660--670},
  year={1944},
  publisher={Taylor \& Francis}
}
@article{hager1989updating,
  author = {Hager, William W},
  title = {Updating the inverse of a matrix},
  journal = {SIAM Review},
  volume = {31},
  number = {2},
  pages = {221--239},
  year = {1989},
}
@article{xu2016least,
	title={Least squares twin support vector machine with universum data for classification},
	author={Xu, Yitian and Chen, Mei and Li, Guohui},
	journal={International Journal of Systems Science},
	volume={47},
	number={15},
	pages={3637--3645},
	year={2016},
	publisher={Taylor \& Francis}
}

@article{xu2012weighted,
	title={A weighted twin support vector regression},
	author={Xu, Yitian and Wang, Laisheng},
	journal={Knowledge-Based Systems},
	volume={33},
	pages={92--101},
	year={2012},
	publisher={Elsevier}
}
@article{shao2013varepsilon,
	title={An $\varepsilon$-twin support vector machine for regression},
	author={Shao, Yuan-Hai and Zhang, Chun-Hua and Yang, Zhi-Min and Jing, Ling and Deng, Nai-Yang},
	journal={Neural Computing and Applications},
	volume={23},
	number={1},
	pages={175--185},
	year={2013},
	publisher={Springer}
}
@article{chen2014improved,
	title={An improved robust and sparse twin support vector regression via linear programming},
	author={Chen, Xiaobo and Yang, Jian and Chen, Long},
	journal={Soft Computing},
	volume={18},
	number={12},
	pages={2335--2348},
	year={2014},
	publisher={Springer}
}
@article{chen2012smooth,
	title={Smooth twin support vector regression},
	author={Chen, Xiaobo and Yang, Jian and Liang, Jun and Ye, Qiaolin},
	journal={Neural Computing and Applications},
	volume={21},
	number={3},
	pages={505--513},
	year={2012},
	publisher={Springer}
}
@article{zhao2013twin,
	title={Twin least squares support vector regression},
	author={Zhao, Yong-Ping and Zhao, Jing and Zhao, Min},
	journal={Neurocomputing},
	volume={118},
	pages={225--236},
	year={2013},
	publisher={Elsevier}
}
@article{zhang2020twin,
	title={Twin Least squares support vector regression of heteroscedastic Gaussian noise model},
	author={Zhang, Shiguang and Liu, Chao and Zhou, Ting and Sun, Lin},
	journal={IEEE Access},
	volume={8},
	pages={94076--94088},
	year={2020},
	publisher={IEEE}
}

@article{demvsar2006statistical,
	title={Statistical comparisons of classifiers over multiple data sets},
	author={Dem{\v{s}}ar, Janez},
	journal={The Journal of Machine Learning Research},
	volume={7},
	pages={1--30},
	year={2006},
	publisher={JMLR. org}
}
@article{chen2012flexible,
	title={A flexible support vector machine for regression},
	author={Chen, Xiaobo and Yang, Jian and Liang, Jun},
	journal={Neural Computing and Applications},
	volume={21},
	number={8},
	pages={2005--2013},
	year={2012},
	publisher={Springer}
}


@article{scholkopf2000new,
 author = "Sch{\"o}lkopf, Bernhard and Smola, Alex J and Williamson, Robert C and Bartlett, Peter L",
 title = {New support vector algorithms},
 journal = {Neural Computation},
 volume = {12},
 number = {5},
 pages = {1207-1245},
 year = {2000},
}

@book{boyd2004convex,
  title = "Convex Optimization",
  author = "Boyd, Stephen and Vandenberghe, Lieven",
  year = "2004",
  publisher = "Cambridge University Press",
}

@incollection{vapnik1998support,
 title = "The support vector method of function estimation",
 author = "Vapnik, Vladimir",
 editor = "Johan A. K. Suykens and Joos Vandewalle",
 booktitle = "Nonlinear Modeling",
 publisher = "Springer",
 address = "Boston, MA",
 pages = "55-85",
 year = "1998",
}
@article{bi2003geometric,
	title={A geometric approach to support vector regression},
	author={Bi, Jinbo and Bennett, Kristin P},
	journal={Neurocomputing},
	volume={55},
	number={1-2},
	pages={79--108},
	year={2003},
	publisher={Elsevier}
}









@article{yang2016laplacian,
	title={Laplacian twin parametric-margin support vector machine for semi-supervised classification},
	author={Yang, Zhiji and Xu, Yitian},
	journal={Neurocomputing},
	volume={171},
	pages={325--334},
	year={2016},
	publisher={Elsevier}
}
@article{yang2018safe,
	title={A safe sample screening rule for Laplacian twin parametric-margin support vector machine},
	author={Yang, Zhiji and Xu, Yitian},
	journal={Pattern Recognition},
	volume={84},
	pages={1--12},
	year={2018},
	publisher={Elsevier}
}


@article{richhariya2021fuzzy,
  title={A fuzzy universum least squares twin support vector machine ({FULSTSVM})},
  author={Richhariya, B and Tanveer, M},
  journal={Neural Computing and Applications},
  pages={1--12},
  year={2021},
  publisher={Springer}
}



@article{angulo2003k,
	title={{K-SVCR}. {A} support vector machine for multi-class classification},
	author={Angulo, Cecilio and Parra, Xavier and Catala, Andreu},
	journal={Neurocomputing},
	volume={55},
	number={1-2},
	pages={57--77},
	year={2003},
	publisher={Elsevier}
}
@article{artacho2018accelerating,
	title={Accelerating the {DC} algorithm for smooth functions},
	author={Artacho, Francisco J Arag{\'o}n and Fleming, Ronan MT and Vuong, Phan T},
	journal={Mathematical Programming},
	volume={169},
	number={1},
	pages={95--118},
	year={2018},
	publisher={Springer}
}
@article{amin2018performance,
	title={Performance evaluation of supervised machine learning classifiers for predicting healthcare operational decisions},
	author={Amin, M and Ali, Amir},
	journal={Wavy AI Research Foundation: Lahore, Pakistan},
	year={2018}
}
@article{ayres2000sisporto,
	title={SisPorto 2.0: a program for automated analysis of cardiotocograms},
	author={Ayres-de-Campos, Diogo and Bernardes, Joao and Garrido, Antonio and Marques-de-Sa, Joaquim and Pereira-Leite, Luis},
	journal={Journal of Maternal-Fetal Medicine},
	volume={9},
	number={5},
	pages={311--318},
	year={2000},
	publisher={Taylor \& Francis}
}
@article{bazikar2020dc,
 author = {Bazikar, Fatemeh and Ketabchi, Saeed and Moosaei, Hossein},
 title = "{DC} programming and {DCA} for parametric-margin $\nu$-support vector machine",
 journal = {Applied Intelligence},
 volume = {50},
 number = {6},
 pages = {1763-1774},
 year = {2020},
}
@article{moosaei2021DC,
 author = "Hossein Moosaei and Fatemeh Bazikar and Saeed Ketabchi and Milan Hlad\'{\i}k",
 title = "Universum parametric-margin $\nu$-support vector machine for classification using the difference of convex functions algorithm",
 journal = "Appl. Intell.",
 fjournal = "Applied Intelligence",
 volume = "52",
 number = "3",
 pages = "2634-2654",
 year = "2022",
}

@inproceedings{bennett2000duality,
	title={Duality and geometry in {SVM} classifiers},
	author={Bennett, Kristin P and Bredensteiner, Erin J},
	volume={2000},
	pages={57--64},
	year={2000},
	publisher = {Morgan Kaufmann Publishers Inc.},
    address = {San Francisco, CA, USA},
    booktitle = {Proceedings of the Seventeenth International    Conference on Machine Learning},
    series = {ICML},
}
@article{tang2021valley,
  title={Valley-loss regular simplex support vector machine for robust multiclass classification},
  author={Tang, Long and Tian, Yingjie and Li, Wenjun and Pardalos, Panos M},
  journal={Knowledge-Based Systems},
  volume={216},
  pages={106801},
  year={2021},
  publisher={Elsevier}
}
@article{tang2020structural,
  title={Structural improved regular simplex support vector machine for multiclass classification},
  author={Tang, Long and Tian, Yingjie and Li, Wenjun and Pardalos, Panos M},
  journal={Applied Soft Computing},
  volume={91},
  pages={106235},
  year={2020},
  publisher={Elsevier}
}
@article{tang2019novel,
  title={A novel perspective on multiclass classification: Regular simplex support vector machine},
  author={Tang, Long and Tian, Yingjie and Pardalos, Panos M},
  journal={Information Sciences},
  volume={480},
  pages={324--338},
  year={2019},
  publisher={Elsevier}
}
@article{tang2018ramp,
  title={Ramp-loss nonparallel support vector regression: robust, sparse and scalable approximation},
  author={Tang, Long and Tian, Yingjie and Yang, Chunyan and Pardalos, Panos M},
  journal={Knowledge-Based Systems},
  volume={147},
  pages={55--67},
  year={2018},
  publisher={Elsevier}
}
@article{moosaei2021,
  title={Generalized Twin Support Vector Machines},
  author={Moosaei, Hossein and Ketabchi, Saeed and Razzaghi, Mohamad and Tanveer, Muhammad},
  journal={Neural Processing Letters},
  volume={53},
  number={2},
  pages={1545--1564},
  year={2021},
  publisher={Springer}
}
@book{boydconvex,
  title={Convex Optimization},
  author={Boyd, Stephen  and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge University Press}
}
@article{bradley2000massive,
	title={Massive data discrimination via linear support vector machines},
	author={Bradley, P S and Mangasarian, O L},
	journal={Optimization Methods and Software},
	volume={13},
	number={1},
	pages={1--10},
	year={2000},
	publisher={Taylor \& Francis}
}
@article{burges1998tutorial,
	title={A tutorial on support vector machines for pattern recognition},
	author={Burges, Christopher J C},
	journal={Data Mining and Knowledge Discovery},
	volume={2},
	number={2},
	pages={121--167},
	year={1998},
	publisher={Springer}
}
@article{belghiti2007new,
	title={A new efficient algorithm based on {DC} programming and {DCA} for clustering},
	author={Belghiti, M Tayeb and Tao, Pham Dinh and others},
	journal={Journal of Global Optimization},
	volume={37},
	number={4},
	pages={593--608},
	year={2007},
	publisher={Springer}
}


@book{cherkassky2007learning,
	title={Learning from Data: Concepts, Theory, and Methods},
	author={Cherkassky, Vladimir and Mulier, Filip M},
	year={2007},
	publisher={Wiley}
}
@book{clarke1990optimization,
	title={Optimization and Nonsmooth Analysis},
	author={Clarke, Frank H},
	year={1990},
	publisher={SIAM}
}

@article{daniel1990friedman,
	title={Friedman two-way analysis of variance by ranks},
	author={Daniel, Wayne W},
	journal={Applied Nonparametric Statistics},
	pages={262--274},
	year={1990},
	publisher={PWS-Kent Boston}
}
@article{ding2017wavelet,
	title={Wavelet twin support vector machines based on glowworm swarm optimization},
	author={Ding, Shifei and An, Yuexuan and Zhang, Xiekai and Wu, Fulin and Xue, Yu},
	journal={Neurocomputing},
	volume={225},
	pages={157--163},
	year={2017},
	publisher={Elsevier}
}
@article{friedman1940comparison,
	title={A comparison of alternative tests of significance for the problem of $m$ rankings},
	author={Friedman, Milton},
	journal={Annals of Mathematical Statistics},
	volume={11},
	number={1},
	pages={86--92},
	year={1940},
	publisher={JSTOR}
}
@article{hao2010new,
	title={New support vector algorithms with parametric insensitive/margin model},
	author={Hao, Pei-Yi},
	journal={Neural Networks},
	volume={23},
	number={1},
	pages={60--73},
	year={2010},
	publisher={Elsevier}
}
@article{hiriart1984generalized,
	title={Generalized {Hessian} matrix and second-order optimality conditions for problems with {$C^{1,1}$} data},
	author={Hiriart-Urruty, Jean-Baptiste and Strodiot, Jean-Jacques and Nguyen, V Hien},
	journal={Applied Mathematics and Optimization},
	volume={11},
	number={1},
	pages={43--56},
	year={1984},
	publisher={Springer}
}
@book{horst2000introduction,
	title={Introduction to Global Optimization},
	author={Horst, Reiner and Pardalos, Panos M and Van Thoai, Nguyen},
	year={2000},
	publisher={Springer}
}
@article{hong1991optimal,
	title={Optimal discriminant plane for a small number of samples and design method of classifier on the plane},
	author={Hong, Zi-Quan and Yang, Jing-Yu},
	journal={Pattern Recognition},
	volume={24},
	number={4},
	pages={317--324},
	year={1991},
	publisher={Elsevier}
}
@article{iman1980approximations,
	title={Approximations of the critical region of the fbietkan statistic},
	author={Iman, Ronald L and Davenport, James M},
	journal={Communications in Statistics-Theory and Methods},
	volume={9},
	number={6},
	pages={571--595},
	year={1980},
	publisher={Taylor \& Francis}
}
@article{karasuyama2012multi,
	title={Multi-parametric solution-path algorithm for instance-weighted support vector machines},
	author={Karasuyama, Masayuki and Harada, Naoyuki and Sugiyama, Masashi and Takeuchi, Ichiro},
	journal={Machine learning},
	volume={88},
	number={3},
	pages={297--330},
	year={2012},
	publisher={Springer}
}

@article{ketabchi2012minimum,
	title={Minimum norm solution to the absolute value equation in the convex case},
	author={Ketabchi, Saeed and Moosaei, Hossein},
	journal={Journal of Optimization Theory and Applications},
	volume={154},
	number={3},
	pages={1080--1087},
	year={2012},
	publisher={Springer}
}


@article{khozeimeh2017expert,
	title={An expert system for selecting wart treatment method},
	author={Khozeimeh, Fahime and Alizadehsani, Roohallah and Roshanzamir, Mohamad and Khosravi, Abbas and Layegh, Pouran and Nahavandi, Saeid},
	journal={Computers in Biology and Medicine},
	volume={81},
	pages={167--175},
	year={2017},
	publisher={Elsevier}
}
@article{khozeimeh2017intralesional,
	title={Intralesional immunotherapy compared to cryotherapy in the treatment of warts},
	author={Khozeimeh, Fahime and Jabbari Azad, Farahzad and Mahboubi Oskouei, Yaghoub and Jafari, Majid and Tehranian, Shahrzad and Alizadehsani, Roohallah and Layegh, Pouran},
	journal={International Journal of Dermatology},
	volume={56},
	number={4},
	pages={474--478},
	year={2017},
	publisher={Wiley Online Library}
}
@article{koczkodaj2017reduce,
	title={How to reduce the number of rating scale items without predictability loss?},
	author={Koczkodaj, Waldemar W and Kakiashvili, Tamar and Szyma{\'n}ska, A and Montero-Marin, J and Araya, Ricardo and Garcia-Campayo, Javier and Rutkowski, Krzysztof and Strza{\l}ka, D},
	journal={Scientometrics},
	volume={111},
	number={2},
	pages={581--593},
	year={2017},
	publisher={Springer}
}
@article{le2011properties,
	title={Properties of two {DC} algorithms in quadratic programming},
	author={Le Thi, Hoai An and Dinh, Tao Pham and Yen, Nguyen Dong},
	journal={Journal of Global Optimization},
	volume={49},
	number={3},
	pages={481--495},
	year={2011},
	publisher={Springer}
}
@article{le2018dc,
	title={{DC} programming and {DCA}: thirty years of developments},
	author={Le Thi, Hoai An and Dinh, Tao Pham},
	journal={Mathematical Programming},
	volume={169},
	number={1},
	pages={5--68},
	year={2018},
	publisher={Springer}
}
@inproceedings{lee2001rsvm,
	title={{RSVM}: Reduced support vector machines},
	author={Lee, Yuh-Jye and Mangasarian, Olvi L},
	booktitle={Proceedings of the 2001 SIAM International Conference on Data Mining},
	pages={1--17},
	year={2001},
	organization={SIAM}
}

@article{de2018improvements,
	title={Improvements on least squares twin multi-class classification support vector machine},
	author={de Lima, M{\'a}rcio Dias and Costa, Nattane Luiza and Barbosa, Rommel},
	journal={Neurocomputing},
	volume={313},
	pages={196--205},
	year={2018},
	publisher={Elsevier}
}
@inproceedings{mayoraz1999support,
	title={Support vector machines for multi-class classification},
	author={Mayoraz, Eddy and Alpaydin, Ethem},
	booktitle={International Work-Conference on Artificial Neural Networks},
	pages={833--842},
	year={1999},
	organization={Springer}
}
@article{melki2018ollawv,
	title={{OLLAWV}: online learning algorithm using worst-violators},
	author={Melki, Gabriella and Kecman, Vojislav and Ventura, Sebastian and Cano, Alberto},
	journal={Applied Soft Computing},
	volume={66},
	pages={384--393},
	year={2018},
	publisher={Elsevier}
}
@misc{musicant1998ndc,
	title={{NDC}: normally distributed clustered datasets},
	institution ="Computer Sciences Department, University of Wisconsin, Madison",
	author={Musicant, D},
	year={1998}
}
@misc{frank2010uci, 
title="{UCI} machine learning repository", 
author={Dua, Dheeru and Graff, Casey}, 
url={https://archive.ics.uci.edu/ml}, 
year={2019}
}
volume={37}, 


@misc{NDCMoosaei,
  title={MC-NDC: multi-class normally distributed clustered datasets. Carleton College, University of Bojnord},
  author={Moosaei, H and Musicant, D and Khosravi, S and Hlad{\'\i}k, M},
  year={2020}
}


@article{pardalos2014minimum,
	title={Minimum norm solution to the positive semidefinite linear complementarity problem},
	author={Pardalos, Panos M and Ketabchi, Saeed and Moosaei, Hossein},
	journal={Optimization},
	volume={63},
	number={3},
	pages={359--369},
	year={2014},
	publisher={Taylor \& Francis}
}
@article{patricio2018using,
	title={Using Resistin, glucose, age and {BMI} to predict the presence of breast cancer},
	author={Patr{\'\i}cio, Miguel and Pereira, Jos{\'e} and Cris{\'o}stomo, Joana and Matafome, Paulo and Gomes, Manuel and Sei{\c{c}}a, Raquel and Caramelo, Francisco},
	journal={BMC cancer},
	volume={18},
	number={1},
	pages={29},
	year={2018},
	publisher={Springer}
}
@article{peng2011tpmsvm,
	title={{TPMSVM}: a novel twin parametric-margin support vector machine for pattern recognition},
	author={Peng, Xinjun},
	journal={Pattern Recognition},
	volume={44},
	number={10-11},
	pages={2678--2692},
	year={2011},
	publisher={Elsevier}
}
@article{qi2012twin,
	title={Twin support vector machine with universum data},
	author={Qi, Zhiquan and Tian, Yingjie and Shi, Yong},
	journal={Neural Networks},
	volume={36},
	pages={112--119},
	year={2012},
	publisher={Elsevier}
}
@book{scholkopf2002learning,
	title={Learning with Kernels: Support Vector Machines, Regularization, Optimization, and Beyond},
	author={Sch{\"o}lkopf, Bernhard and Smola, Alexander J and Bach, Francis and others},
	year={2002},
	publisher={MIT Press}
}
@article{khozeimeh2021combining,
  title={Combining a convolutional neural network with autoencoders to predict the survival chance of {COVID}-19 patients},
  author={Khozeimeh, Fahime and Sharifrazi, Danial and Izadi, Navid Hoseini and Joloudari, Javad Hassannataj and Shoeibi, Afshin and Alizadehsani, Roohallah and Gorriz, Juan M and Hussain, Sadiq and Sani, Zahra Alizadeh and Moosaei, Hossein and others},
  journal={Scientific Reports},
  volume={11},
  number={1},
  pages={1--18},
  year={2021},
  publisher={Nature Publishing Group}
}

@inproceedings{sinz2007analysis,
  title={An Analysis of Inference with the Universum.},
  author={Sinz, Fabian H and Chapelle, Olivier and Agarwal, Alekh and Sch{\"o}lkopf, Bernhard},
  booktitle={Advances in Neural Information Processing Systems},
  volume={7},
  pages={1369--1376},
  year={2008}
}

 @article{tanveer2016robust,
	title={Robust energy-based least squares twin support vector machines},
	author={Tanveer, Mohammad and Khan, Mohammad Asif and Ho, Shen-Shyang},
	journal={Applied Intelligence},
	volume={45},
	number={1},
	pages={174--186},
	year={2016},
	publisher={Springer}
}
@article{tao1996numerical,
	title={Numerical solution for optimization over the efficient set by dc optimization algorithms},
	author={Tao, Pham Dinh and others},
	journal={Operations Research Letters},
	volume={19},
	number={3},
	pages={117--128},
	year={1996},
	publisher={Elsevier}
}
@book{vapnik1974theory,
	title={Theory of Pattern Recognition},
	author={Vapnik, Vladimir and Chervonenkis, Alexey},
	year={1974},
	publisher={Nauka, Moscow}
}
@book{vapnik2013nature,
	title={The Nature of Statistical Learning Theory},
	author={Vapnik, Vladimir},
	year={2013},
	publisher={Springer}
}
@article{mei2019multi,
  title={Multi-task least squares twin support vector machine for classification},
  author={Mei, Benshan and Xu, Yitian},
  journal={Neurocomputing},
  volume={338},
  pages={26--33},
  year={2019},
  publisher={Elsevier}
}
@inproceedings{wang2021data,
	title={Data Science for Characterizing Breast Cancer},
	author={Wang, Lingxiao},
	booktitle={2021 3rd International Conference on Intelligent Medicine and Image Processing},
	pages={122--126},
	year={2021}
}
@article{wang2018improved,
	title={An improved $\nu$-twin bounded support vector machine},
	author={Wang, Huiru and Zhou, Zhijian and Xu, Yitian},
	journal={Applied Intelligence},
	volume={48},
	number={4},
	pages={1041--1053},
	year={2018},
	publisher={Springer}
}
@inproceedings{weston2006inference,
	title={Inference with the universum},
	author={Weston, Jason and Collobert, Ronan and Sinz, Fabian and Bottou, L{\'e}on and Vapnik, Vladimir},
	booktitle={Proceedings of the 23rd International Conference on Machine Learning},
	pages={1009--1016},
	year={2006}
}
@article{xu2016k,
	title={K-nearest neighbor-based weighted multi-class twin support vector machine},
	author={Xu, Yitian},
	journal={Neurocomputing},
	volume={205},
	pages={430--438},
	year={2016},
	publisher={Elsevier}
}

@inproceedings{zhang2015sparse,
 author = "LeCun, Yann and Boser, Bernhard E and Denker, John S and Henderson, Donnie and Howard, Richard E and Hubbard, Wayne E and Jackel, Lawrence D",
 title = "Handwritten digit recognition with a back-propagation network",
 editor = "David S. Touretzky",
 booktitle = "Advances in Neural Information Processing Systems 2",
 publisher = "Morgan Kaufmann Publishers Inc.",
 pages = "396-404",
 year = "1990",
}
@article{Tao,
  title={A convex optimization approach for minimizing the ratio of indefinite quadratic functions over an ellipsoid},
  author={Beck, Amir and Teboulle, Marc},
  journal={Mathematical Programming},
  volume={118},
  number={1},
  pages={13--35},
  year={2009},
  publisher={Springer}
}

@book{V,
  title={Nonlinear Programming: Theory and Algorithms},
  author={Bazaraa, Mokhtar S and Sherali, Hanif D and Shetty, Chitharanjan M},
  year={2013},
  publisher={Wiley}
}

@techreport{xz,
  title={Complementary pivot theory of mathematical programming},
  author={Cottle, Richard W and Dantzig, George B},
  year={1967},
  institution={STANFORD UNIV CA OPERATIONS RESEARCH HOUSE}
}
@article{cottle1967complementary,
	author = "Cottle, Richard W. and Dantzig, George B.",
	journal = "Linear Algebra and its Applications",
	number = "1",
	pages = "103--125",
	title = "{Complementary pivot theory of mathematical programming}",
	volume = "1",
	year = "1968",
}



@book{bertsekas1999nonlinear,
  title={Nonlinear Programming},
  publisher = {Athena Scientific},
  address = {Belmont, MA},
  edition = {2nd}, 
  author={Bertsekas, DP},
  year={1999}
}

@book{cottle1992linear,
  title={The Linear Complementarity Problem},
  author={Cottle, Richard W and Pang, Jong-Shi and Stone, Richard E},
  publisher = {Academic Press},
  address={Boston, MA},
  year={1992}
}

@incollection{evtushenko2003new,
  title={New perspective on the theorems of alternative},
  author={Evtushenko, Yu G and Golikov, AI},
  booktitle={High Performance Algorithms and Software for Nonlinear Optimization},
  pages={227--241},
  year={2003},
  publisher={Springer}
}

@article{kanzow2003minimum,
  title={On the minimum norm solution of linear programs},
  author={Kanzow, Christian and Qi, Houduo and Qi, Liqun},
  journal={Journal of Optimization Theory and Applications},
  volume={116},
  number={2},
  pages={333--345},
  year={2003},
  publisher={Springer}
}

@article{ketabchi2007solution,
  title={On the solution set of convex problems and its numerical application},
  author={Ketabchi, S and Ansari-Piri, E},
  journal={Journal of Computational and Applied Mathematics},
  volume={206},
  number={1},
  pages={288--292},
  year={2007},
  publisher={North-Holland}
}

@article{mangasarian1988simple,
  title={A simple characterization of solution sets of convex programs},
  author={Mangasarian, Olvi L},
  journal={Operations Research Letters},
  volume={7},
  number={1},
  pages={21--26},
  year={1988},
  publisher={Elsevier}
}

@article{mangasarian2004newton,
  title={A {Newton} method for linear programming},
  author={Mangasarian, OL},
  journal={Journal of Optimization Theory and Applications},
  volume={121},
  number={1},
  pages={1--18},
  year={2004},
  publisher={Springer}
}

@article{mangasarian2007absolute,
  title={Absolute value programming},
  author={Mangasarian, OL},
  journal={Computational Optimization and Applications},
  volume={36},
  number={1},
  pages={43--53},
  year={2007},
  publisher={Springer}
}


@article{mangasarian2006absolute,
  title={Absolute value equations},
  author={Mangasarian, OL and Meyer, RR},
  journal={Linear Algebra and its Applications},
  volume={419},
  number={2-3},
  pages={359--367},
  year={2006},
  publisher={Elsevier}
}










@book{nocedal2006numerical,
  title={Numerical Optimization},
  author={Nocedal, Jorge and Wright, Stephen},
  year={2006},
  publisher={Springer},
  address = {New York},
}

@book{tikhonov1977solutions,
  title={Solutions of Ill-Posed Problems},
  author={Tikhonov, Andrey N and Arsenin, Vasilii Iakkovlevich},
  year={1977},
  publisher={Winston},
  address={Washington, DC},
}
  volume={14},

@article{golub1999tikhonov,
  title="{Tikhonov} regularization and total least squares",
  author={Golub, Gene H and Hansen, Per Christian and O'Leary, Dianne P},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={21},
  number={1},
  pages={185--194},
  year={1999},
  publisher={SIAM}
}

@article{renaut2004efficient,
  title={Efficient algorithms for solution of regularized total least squares},
  author={Renaut, Rosemary A and Guo, Hongbin},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={26},
  number={2},
  pages={457--476},
  year={2004},
  publisher={SIAM}
}

@article{amaral2005framework,
  title={A framework for optimal correction of inconsistent linear constraints},
  author={Amaral, Paula and Barahona, Pedro},
  journal={Constraints},
  volume={10},
  number={1},
  pages={67--86},
  year={2005},
  publisher={Springer}
}

@article{beck2006solution,
  title={On the solution of the {Tikhonov} regularization of the total least squares problem},
  author={Beck, Amir and Ben-Tal, Aharon},
  journal={SIAM Journal on Optimization},
  volume={17},
  number={1},
  pages={98--118},
  year={2006},
  publisher={SIAM}
}

@article{more1983computing,
  title={Computing a trust region step},
  author={Mor{\'e}, Jorge J and Sorensen, Danny C},
  journal={SIAM Journal on Scientific and Statistical Computing},
  volume={4},
  number={3},
  pages={553--572},
  year={1983},
  publisher={SIAM}
}

@article{mangasarian2009generalized,
  title={A generalized {Newton} method for absolute value equations},
  author={Mangasarian, OL},
  journal={Optimization Letters},
  volume={3},
  number={1},
  pages={101--108},
  year={2009},
  publisher={Springer}
}


@article{rohn2004theorem,
  title={A theorem of the alternatives for the equation {$Ax+ B|x|= b$}},
  author = "Rohn, Ji\v{r}\'{\i}",
  journal={Linear and Multilinear Algebra},
  volume={52},
  number={6},
  pages={421--426},
  year={2004},
  publisher={Taylor \& Francis}
}

@article{prokopyev2009equivalent,
  title={On equivalent reformulations for absolute value equations},
  author={Prokopyev, Oleg},
  journal={Computational Optimization and Applications},
  volume={44},
  number={3},
  pages={363-372},
  year={2009},
  publisher={Springer}
}


@article{ketabchi2012optimal,
  title={Optimal error correction and methods of feasible directions},
  author={Ketabchi, Saeed and Moosaei, Hossein},
  journal={Journal of Optimization Theory and Applications},
  volume={154},
  number={1},
  pages={209--216},
  year={2012},
  publisher={Springer}
}

@book{higham2002accuracy,
  title={Accuracy and Stability of Numerical Algorithms},
  author={Higham, Nicholas J},
  year={2002},
  publisher={SIAM}
}
  volume={80},

@article{hladik2016radii,
  title={Radii of solvability and unsolvability of linear systems},
  author={Hlad{\'\i}k, Milan and Rohn, Ji{\v{r}}{\'\i}},
  journal={Linear Algebra and its Applications},
  volume={503},
  pages={120--134},
  year={2016},
  publisher={Elsevier}
}

@article{markovsky2007overview,
  title={Overview of total least-squares methods},
  author={Markovsky, Ivan and Van Huffel, Sabine},
  journal={Signal Processing},
  volume={87},
  number={10},
  pages={2283--2302},
  year={2007},
  publisher={Elsevier}
}

@book{van1991total,
  title={The Total Least Squares Problem: Computational Aspects and Analysis},
  author={Van Huffel, Sabine and Vandewalle, Joos},
  volume={9},
  year={1991},
  publisher={SIAM}
}

@article{moosaei2015some,
  title={Some techniques for solving absolute value equations},
  author={Moosaei, Hossein and Ketabchi, Saeed and Noor, Muhammad Aslam and Iqbal, Javed and Hooshyarbakhsh, Vahideh},
  journal={Applied Mathematics and Computation},
  volume={268},
  pages={696--705},
  year={2015},
  publisher={Elsevier}
}

@article{hu2010note,
  title={A note on absolute value equations},
  author={Hu, Sheng-Long and Huang, Zheng-Hai},
  journal={Optimization Letters},
  volume={4},
  number={3},
  pages={417--424},
  year={2010},
  publisher={Springer}
}

@article{mangasarian2014linear,
  title={Linear complementarity as absolute value equation solution},
  author={Mangasarian, Olvi L},
  journal={Optimization Letters},
  volume={8},
  number={4},
  pages={1529--1534},
  year={2014},
  publisher={Springer}
}

@article{rohn2014iterative,
  title={An iterative method for solving Absolute value equations and sufficient conditions for unique solvability},
  author={Rohn, Ji\v{r}\'{\i} and Hooshyarbakhsh, Vahideh and Farhadsefat, Raena},
  journal={Optimization Letters},
  volume={8},
  number={1},
  pages={35--44},
  year={2014},
  publisher={Springer}
}

@article{iqbal2015levenberg,
  title={{Levenberg}--{Marquardt} method for solving systems of absolute value equations},
  author={Iqbal, Javed and Iqbal, Asif and Arif, Muhammad},
  journal={Journal of Computational and Applied Mathematics},
  volume={282},
  pages={134--138},
  year={2015},
  publisher={Elsevier}
}
@article{mangasarian2015hybrid,
  title={A hybrid algorithm for solving the absolute value equation},
  author={Mangasarian, Olvi L},
  journal={Optimization Letters},
  volume={9},
  number={7},
  pages={1469--1474},
  year={2015},
  publisher={Springer}
}

@article{hladik2018bounds,
  title={Bounds for the solutions of absolute value equations},
  author={Hlad{\'\i}k, Milan},
  journal={Computational Optimization and Applications},
  volume={69},
  number={1},
  pages={243--266},
  year={2018},
  publisher={Springer}
}

@article{rohn2009unique,
  title={On unique solvability of the absolute value equation},
  author={Rohn, Ji\v{r}\'{\i}},
  journal={Optimization Letters},
  volume={3},
  number={4},
  pages={603--606},
  year={2009},
  publisher={Springer}
}

@article{wu2016unique,
  title={On the unique solvability of the absolute value equation},
  author={Wu, Shi-Liang and Guo, Peng},
  journal={Journal of Optimization Theory and Applications},
  volume={169},
  number={2},
  pages={705--712},
  year={2016},
  publisher={Springer}
}

@article{ketabchi2012efficient,
  title={An efficient method for optimal correcting of absolute value equations by minimal changes in the right hand side},
  author={Ketabchi, Saeed and Moosaei, Hossein},
  journal={Computers \& Mathematics with Applications},
  volume={64},
  number={6},
  pages={1882--1885},
  year={2012},
  publisher={Elsevier}
}

@article{ketabchi2013optimal,
  title={Optimal error correction of the absolute value equation using a genetic algorithm},
  author={Ketabchi, Saeed and Moosaei, Hossein and Fallahi, Saeed},
  journal={Mathematical and Computer Modelling},
  volume={57},
  number={9-10},
  pages={2339--2342},
  year={2013},
  publisher={Elsevier}
}

@article{moosaei2016tikhonov,
  title={Tikhonov regularization for infeasible absolute value equations},
  author={Moosaei, Hossein and Ketabchi, Saeed and Pardalos, Panos M},
  journal={Optimization},
  volume={65},
  number={8},
  pages={1531--1537},
  year={2016},
  publisher={Taylor \& Francis}
}
@article{moosaei2015minimum,
  title={Minimum norm solution of the absolute value equations via simulated annealing algorithm},
  author={Moosaei, Hossein and Ketabchi, Saeed and Jafari, Hamed},
  journal={Afrika Matematika},
  volume={26},
  number={7-8},
  pages={1221--1228},
  year={2015},
  publisher={Springer}
}

@article{amaral2005connections,
  title={Connections between the total least squares and the correction of an infeasible system of linear inequalities},
  author={Amaral, Paula and Barahona, Pedro},
  journal={Linear Algebra and its Applications},
  volume={395},
  pages={191--210},
  year={2005},
  publisher={Elsevier}
}
@article{amaral2009optimal,
  title={On optimal zero-preserving corrections for inconsistent linear systems},
  author={Amaral, Paula and Fernandes, Lu{\'\i}s M and J{\'u}dice, Joaquim and Sherali, Hanif D},
  journal={Journal of Global Optimization},
  volume={45},
  number={4},
  pages={645--666},
  year={2009},
  publisher={Springer}
}

@article{salahi2010correcting,
  title={Correcting an inconsistent set of linear inequalities by the generalized {Newton} method},
  author={Salahi, Maziar and Ketabchi, Saeed},
  journal={Optimization Methods \& Software},
  volume={25},
  number={3},
  pages={457--465},
  year={2010},
  publisher={Taylor \& Francis}
}

@article{rohn1989systems,
  title={Systems of linear interval equations},
 author = "Rohn, Ji\v{r}\'{\i}",
  journal={Linear Algebra and its Applications},
  volume={126},
  pages={39--78},
  year={1989},
  publisher={Elsevier}
}

@article{rohn1984solving2,
  title={Proofs to '{Solving} Interval Linear Systems'},
  author={Rohn, Ji{\v{r}}{\'\i}},
  year={1984},
  publisher={Inst. f. Angewandte Mathematik, Univ.}
}

@techReport{rohn1984solving,
 author = "Rohn, Ji\v{r}\'{\i}",
 title = "Proofs to 'Solving Interval Linear Systems'",
 type = " Freiburger Intervall-Berichte",
 number = "84/7",
 pages = "17-30",
 year = "1984",
 institution = "Albert-Ludwigs-Universit{\"a}t",
 address = "Freiburg",
}


@book{bjorck1996numerical,
  title={Numerical Methods for Least Squares Problems},
  author={Bj{\"o}rck, {$\AA$}ke},
  year={1996},
  publisher={SIAM}
}
@book{brezis1999analyse,
  title={Analyse fonctionnelle: th{\'e}orie et applications},
  author={Brezis, Ha{\"\i}m and Ciarlet, Philippe G and Lions, Jacques Louis},
  volume={91},
  year={1999},
  publisher={Dunod Paris}
}

@article{sherali1992global,
  title={A global optimization algorithm for polynomial programming problems using a reformulation-linearization technique},
  author={Sherali, Hanif D and Tuncbilek, Cihan H},
  journal={Journal of Global Optimization},
  volume={2},
  number={1},
  pages={101--112},
  year={1992},
  publisher={Springer}
}
@book{david2008linear,
  title={Linear and nonlinear programming},
  author={David G, Luenberger and Ye, Yinyu},
  year={2008},
  publisher={New York, NY: Springer,}
}
@incollection{gauvin1982differential,
  title={Differential properties of the marginal function in mathematical programming},
  author={Gauvin, Jacques and Dubeau, Fran{\c{c}}ois},
  editor = "Guignard, Monique",
  booktitle={Optimality and Stability in Mathematical Programming},
  pages={101--119},
  year={1982},
  publisher={Springer},
   volume = "19",
   series = "Mathematical Programming Studies",
}

@article{raayatpanah2019absolute,
  title={Absolute value equations with uncertain data},
  author={Raayatpanah, M.A. and Moosaei, H. and Pardalos, P.M.},
  journal={Optimization Letters},
  pages={1--12},
  year={2019},
   note = "in presss",
}
@unpublished{ZamHla2020aa,
 author = "Moslem Zamani and Milan Hlad\'{\i}k",
 title = "Error bounds and a condition number for the absolute value equations",
 url = "https://arxiv.org/abs/1912.12904",
 note = "preprint arXiv: 1912.12904",
 year = "2020",
}
@article{zhao2019improved,
	title={An improved non-parallel Universum support vector machine and its safe sample screening rule},
	author={Zhao, Jiang and Xu, Yitian and Fujita, Hamido},
	journal={Knowledge-Based Systems},
	volume={170},
	pages={79--88},
	year={2019},
	publisher={Elsevier}
}
@article{xiao2020new,
 author = {Xiao, Yanshan and Wen, Jing and Liu, Bo},
 title = {A new multi-task learning method with universum data},
 journal = {Applied Intelligence},
 volume = {51},
 pages = {3421-3434},
 year = {2021},
}
@article{fukushima1981generalized,
	title={A generalized proximal point algorithm for certain non-convex minimization problems},
	author={Fukushima, Masao and Mine, Hisashi},
	journal={International Journal of Systems Science},
	volume={12},
	number={8},
	pages={989--1000},
	year={1981},
	publisher={Taylor \& Francis}
}
@article{li2018face,
 author={Li, Meijing and Yu, Xiuming and Ryu, Keun Ho and Lee, Sanghyuk and Theera-Umpon, Nipon},
 title={Face recognition technology development with {Gabor}, {PCA} and {SVM} methodology under illumination normalization condition},
 journal={Cluster Computing},
 volume={21},
 number={1},
 pages={1117-1126},
 year={2018},
}
@article{tanveer2020machine,
  title={Machine learning techniques for the diagnosis of Alzheimer’s disease: A review},
  author={Tanveer, M and Richhariya, B and Khan, RU and Rashid, AH and Khanna, P and Prasad, M and Lin, CT},
  journal={ACM Transactions on Multimedia Computing, Communications, and Applications (TOMM)},
  volume={16},
  number={1s},
  pages={1--35},
  year={2020},
  publisher={ACM New York, NY, USA}
}
@article{AARM,
  title={Computer aided decision making for heart disease detection using hybrid neural network-Genetic algorithm},
  author={Arabasadi, Zeinab and Alizadehsani, Roohallah and Roshanzamir, Mohamad and Moosaei, Hossein and Yarifard, Ali Asghar},
  journal={Computer methods and programs in biomedicine},
  volume={141},
  pages={19--26},
  year={2017},
  publisher={Elsevier}
}
@incollection{GT,
  title={Optimization Techniques for Date Representions with Biomedical Applications},
  author={Georgiev, Pando G and Theis, Fabian J},
  booktitle={Handbook of Optimization in Medicine},
  pages={1--38},
  year={2009},
  publisher={Springer}
}
@inCollection{noble2004support,
 author = "Noble, William Stafford and others",
 title = "Support vector machine applications in computational biology",
 editor = "B. Schoelkopf, K. Tsuda and J.-P. Vert",
 booktitle = "Kernel Methods in Computational Biology",
 publisher = "MIT Press",
 series = "Computational Molecular Biology",
 pages = "71-92",
 year = "2004",
}

@article{chicco2017ten,
  title={Ten quick tips for machine learning in computational biology},
  author={Chicco, Davide},
  journal={BioData mining},
  volume={10},
  number={1},
  pages={35},
  year={2017},
  publisher={Springer}
}


@article{ding2017twin,
  title={Twin support vector machine: theory, algorithm and applications},
  author={Ding, Shifei and Zhang, Nan and Zhang, Xiekai and Wu, Fulin},
  journal={Neural Computing and Applications},
  volume={28},
  number={11},
  pages={3119--3130},
  year={2017},
  publisher={Springer}
}
@article{tian2014review,
  title={Review on: twin support vector machines},
  author={Tian, Yingjie and Qi, Zhiquan},
  journal={Annals of Data Science},
  volume={1},
  number={2},
  pages={253--277},
  year={2014},
  publisher={Springer}
}
@article{artacho2020using,
  title={Using positive spanning sets to achieve d-stationarity with the boosted dc algorithm},
  author={Artacho, FJ Arag{\'o}n and Campoy, Rub{\'e}n and Vuong, Phan T},
  journal={Vietnam Journal of Mathematics},
  volume={48},
  number={2},
  pages={363},
  year={2020},
  publisher={Springer}
}
@article{aragon2020boosted,
  title={The boosted difference of convex functions algorithm for nonsmooth functions},
  author={Arag{\'o}nArtacho, Francisco J and Vuong, Phan T},
  journal={SIAM Journal on Optimization},
  volume={30},
  number={1},
  pages={980--1006},
  year={2020},
  publisher={SIAM}
}
@misc{hsu2003practical,
 title = "A practical guide to support vector classification",
 author = "Hsu, Chih-Wei and Chang, Chih-Chung and Lin, Chih-Jen and others",
 year = "2003",
 address = "Taipei",
 url = "https://www.csie.ntu.edu.tw/~cjlin/papers/guide/guide.pdf",
}

@comment{x-kbibtex-personnameformatting=<%l><, %f>}

@article{FunMan2011,
 author = "Fung, G. M. and Mangasarian, O. L.",
title = "Equivalence of Minimal {$\ell_0$}- and {$\ell_p$}-Norm Solutions of Linear Equalities, Inequalities and Linear Programs for Sufficiently Small {$p$}",
 journal = "Journal of Optimization Theory and Applications",
 number = "1",
 pages = "1-10",
 volume = "151",
 year = "2011",
}



